The CIDA Variability Survey of Orion OB1 II: demographics of the young, low-mass stellar populations

We present results of our large scale, optical, multi-epoch photometric survey of ~180 square degrees across the Orion OB1 association, complemented with extensive follow up spectroscopy. We map and characterize in an uniform way the off-cloud, low-mass, pre-main sequence populations. We report 2064, mostly K and M-type, confirmed T Tauri members. Most (59%) are located in the OB1a subassociation, 27% in OB1b, and 14% within the confines of the A and B molecular clouds. There is significant structure in the spatial distribution of the young stars. We characterize two new clusterings of T Tauri stars, HD 35762 and HR 1833 in the OB1a subassociation, and two stellar overdensities in OB1b. There is indication of two populations of young stars in the OB1b region, located at two different distances, which may be due to the OB1a subassociation overlapping on front of OB1b. The various groups and regions can be ordered in an age sequence that agrees with the long standing picture of star formation starting in Orion OB1a some 10-15 Myr ago. We define a new type of T Tauri star, the C/W class, objects we propose may be nearing the end of their accretion phase. We detect the observational signature of Li depletion in young K and M stars with a timescale of 8.5 Myr. The decline of the accretion fraction from ~2 - 10 Myr, implies an accretion e-folding timescale of 2.1 Myr. Finally, the median amplitude of the V-band variability shows the decline of stellar activity, from accreting Classical T Tauri stars to the least active field dwarfs.

==> comparison_with_other_works.tex <==
\begin {deluxetable*}{llllcccl}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{Comparison with other population studies in Orion OB1 \label{speclog}}
\tablehead{
\colhead{Work} & \colhead{Technique$\rm^{(a)}$} & \colhead{Region} & \colhead{Coverage (Sq.Deg.)} & \colhead{Candidate TTS} & \colhead{Confirmed TTS} & \colhead{Matches with CVSO} \\
}
\startdata
This work              & Optical: P+S &  1a, 1b, A cloud, B cloud &  180       &  11201      & 2064    & 2064 \\
\cite{wiramihardja1989,kogure1989,wiramihardja1991} & Optical: OP & 1a, 1b, A \& B clouds & 100 & 759 & 0 & 102 \\
\cite{hillenbrand1997} & Optical: P+S &  ONC                      &  0.3       &  3500       &  675(b) &  27  \\
\cite{briceno05}       & Optical: P+S &  1a, 1b, B cloud          & 68         &  1403       &  197    & 197  \\
\cite{briceno07b}      & Optical: P+S &  1a                       &  3.1       &   266       &   78    &  78  \\
\cite{vereshchagin2010}& Optical: PM  &  ONC                      &  9         & 13577       &    0    & 170  \\ 
\cite{biazzo2011}      & Optical: S   &  1a                       & \nodata (c)&  \nodata (c)&    8    &   8  \\ 
\cite{vaneyken2011}    & Optical: P   &  1a (25 Ori)              &   0.3      &    16       &    0    &   6  \\
\cite{alves2012}       & Optical: P   &  A-cloud (NGC 1980-ONC)   &  25        &  2336(d)    &    0    & 118  \\
\cite{megeath2012}     & NIR: P       &  A and B clouds           & $\sim 9$   &  2991       &    0    &  82  \\
\cite{da-rio2012}      & Optical: P   &  ONC                      &   0.25     &  1750       &    0    &  26  \\       
\cite{hsu2012}         & Optical: P+S &  A cloud (L1641)          & $\sim 3.2$ &  $\sim 1080$&  864    &  22  \\
\cite{pillitteri2013}  & X-ray: P     &  A cloud (L1641)          & $\sim 2.8$ &   716       &    0    &  16  \\
\cite{hillenbrand2013} & Optical: P+S &  ONC                      &   0.3      &  3500       &  929(e) &  27  \\
\cite{sanchez2014}     & UV: P        &  Orion OB1                & 400        &   111       &    0    &  11  \\   
\cite{spezzi2015}      & NIR: P       &  B cloud (NGC 2068, 2024) &  $\sim 1.6$&   186       &    0    &  10  \\
\cite{da-rio2016}      & NIR: S       &  A cloud                  &  $\sim 6$  &  2691       &    0    & 100  \\
\cite{karim2016}       & Optical: P   &  1a, 1b, A cloud, B cloud &  180       & \nodata (f) & 1974(f) & 1974 \\
\cite{suarez2017}      & Optical: P+S &  1a (25 Ori)              &  $\sim  7$ &   172       &   53    &  25  \\
\cite{kounkel2017b}    & Optical: P+S &  A cloud (NGC 1980)       & $\sim 0.25$&   280       &  148    &   9  \\
\cite{fang2017}        & Optical: P+S &  A cloud (NGC 1980)       & $\sim 5.25$&  1275       &  619    &  24  \\
\enddata                    
\tablecomments{(a) P: Photometry, S:Spectroscopy, OP: Objective prism (slitless spectroscopy);
(b) Objects with a membership probability $\ge 90$ and a spectral type determination;
(c) This study characterized metallicity of targets selected from \cite{briceno07b};
(d) Candidates for which probability of membership was $\ge 99$\%;
(e) \cite{hillenbrand2013} report new spectral typing of 254 stars, which we added to the sample of \cite{hillenbrand1997};
(f) The \cite{karim2016} sample is drawn from the list of CVSO TTS in this work. However, only positions, type (WTTS or CTTS) and
photometric information was provided. Periods were derived for 564 TTS.
}
\end{deluxetable*}


